Interpreting Latent Student Knowledge Representations in Programming Assignments

Recent advances in artificial intelligence for education leverage generative large language models, including using them to predict open-ended student responses rather than their correctness only. However, the black-box nature of these models limits the interpretability of the learned student knowledge representations. In this paper, we conduct a first exploration into interpreting latent student knowledge representations by presenting InfoOIRT, an Information regularized Open-ended Item Response Theory model, which encourages the latent student knowledge states to be interpretable while being able to generate student-written code for open-ended programming questions. InfoOIRT maximizes the mutual information between a fixed subset of latent knowledge states enforced with simple prior distributions and generated student code, which encourages the model to learn disentangled representations of salient syntactic and semantic code features including syntactic styles, mastery of programming skills, and code structures. Through experiments on a real-world programming education dataset, we show that InfoOIRT can both accurately generate student code and lead to interpretable student knowledge representations.

==> student_codes/conciseness_11_original.tex <==
\begin{lstlisting}
public int caughtSpeeding(int speed, boolean isBirthday)
{
    if (isBirthday)
    {
        if (speed <= 65)
        {
            return 0;
        }
        else if (speed >= 66 && speed <= 85)
        {
            return 1;
        }
        else
        {
            return 2;
        }
    }
    else
    {
        if (speed <= 60)
        {
            return 0;
        }
        else if (speed >= 61 && speed <= 80)
        {
            return 1;
        }
        else
        {
            return 2;
        }
    }
}\end{lstlisting}

==> student_codes/conciseness_21.tex <==
\begin{lstlisting}
public int blackjack(int a, int b)
{
    if (a > 21 && b > 21)
    {
        return 0;
    }
    else if (a > 21)
    {
        return b;
    }
    else if (b > 21)
    {
        return a;
    }
    else
    {
        return a;
    }
}\end{lstlisting}

==> student_codes/conciseness_22.tex <==
\begin{lstlisting}
public int blackjack(int a, int b)
{
    if (a > 21 && b > 21)
        return 0;
    else if (a > 21)
        return b;
    else if (b > 21)
        return a;
    else
        return a > b? a : b;
}\end{lstlisting}

==> student_codes/conciseness_31.tex <==
\begin{lstlisting}
public boolean in1To10(int n, boolean outsideMode)
{
    if (outsideMode)
    {
        if (n <= 1 || n >= 10)
        {
            return true;
        }
        else
        {
            return false;
        }
    }
    else
    {
        if (n >= 1 && n <= 10)
        {
            return true;
        }
        else
        {
            return false;
        }
    }
}\end{lstlisting}

==> student_codes/conciseness_32.tex <==
\begin{lstlisting}
public boolean in1To10(int n, boolean outsideMode)
{
    if(outsideMode)
        return (n <= 1 || n >= 10);
    return (n >= 1 && n <= 10);
}\end{lstlisting}

==> student_codes/conciseness_41_original.tex <==
\begin{lstlisting}
public boolean cigarParty(int cigars, boolean isWeekend)
{
    if (isWeekend)
    {
        if (cigars >= 40)
        {
            return true;
        }
        else
        {
            return false;
        }
    }
    else
    {
        if (cigars >= 40 && cigars <= 60)
        {
            return true;
        }
        else
        {
            return false;
        }
    }
}\end{lstlisting}

==> student_codes/problem_type_21.tex <==
\begin{lstlisting}
public int redTicket(int a, int b, int c)
{
    if(a == b && b == c)
    {
        if(a == 2)
            return 10;
        return 5;
    }
    if(a!= b && a!=c)
        return 1;
    return 0;
}\end{lstlisting}

==> student_codes/problem_type_22.tex <==
\begin{lstlisting}
public int[] withoutTen(int[] nums)
{
    int[] arr = new int[nums.length];
    int p = 0;
    for(int i = 0; i < nums.length; i++)
    {
        if(nums[i]!= 10)
        {
            arr[p] = nums[i];
            p++;
        }
    }
    return arr;
}\end{lstlisting}

==> student_codes/problem_type_31.tex <==
\begin{lstlisting}
public String alarmClock(int day, boolean vacation)
{
    if(vacation)
    {
        if(day == 0 || day == 6)
            return "off";
        return "10:00";
    }
    else
    {
        if(day == 0 || day == 6)
            return "10:00";
        return "7:00";
    }
}\end{lstlisting}

==> student_codes/problem_type_32.tex <==
\begin{lstlisting}
public int[] fizzArray(int n)
{
    int[] arr = new int[n];
    
    for(int i = 0; i < n; i++)
        arr[i] = i;
              
    return arr;
}\end{lstlisting}

==> student_codes/style_21.tex <==
\begin{lstlisting}
public int[] frontPiece(int[] nums)
{
    int[] front;
    if (nums.length >= 2) {
        front = new int[2];
        front[0] = nums[0];
        front[1] = nums[1];
    }
    else if (nums.length == 1) {
        front = new int[1];
        front[0] = nums[0];
    }
    else {
        front = new int[0];
    }
    return front;
}\end{lstlisting}

==> student_codes/style_22.tex <==
\begin{lstlisting}
public int[] frontPiece(int[] nums)
{
    int[] front;
    if (nums.length >= 2)
    {
        front = new int[2];
        front[0] = nums[0];
        front[1] = nums[1];
    }
    else if (nums.length == 1)
    {
        front = new int[1];
        front[0] = nums[0];
    }
    else
    {
        front = new int[0];
    }
    return front;
}\end{lstlisting}

==> student_codes/style_31.tex <==
\begin{lstlisting}
public int sum67(int[] nums)
{
    int sum = 0;
    for (int i = 0; i < nums.length; i++) {
        if (nums[i] == 6) {
            while (nums[i]!= 7) {
                i++;
            }
        }
        else {
            sum += nums[i];
        }
    }
    return sum;
}\end{lstlisting}

==> student_codes/style_32.tex <==
\begin{lstlisting}
public int sum67(int[] nums)
{
    int sum = 0;
    for (int i = 0; i < nums.length; i++)
    {
        if (nums[i] == 6)
        {
            for (int j = i; j < nums.length; j++)
            {
                if (nums[j] == 7)
                 {
                     break;
                 }
             }
            else if (nums[j] == 6)
            {
                sum += nums[j];
            }
        }
    }
    return sum;
}\end{lstlisting}
